Ego-Body Pose Estimation via Ego-Head Pose Estimation

Estimating 3D human motion from an egocentric video sequence plays a critical role in human behavior understanding and has various applications in VR/AR. However, naively learning a mapping between egocentric videos and human motions is challenging, because the user's body is often unobserved by the front-facing camera placed on the head of the user. In addition, collecting large-scale, high-quality datasets with paired egocentric videos and 3D human motions requires accurate motion capture devices, which often limit the variety of scenes in the videos to lab-like environments. To eliminate the need for paired egocentric video and human motions, we propose a new method, Ego-Body Pose Estimation via Ego-Head Pose Estimation (EgoEgo), which decomposes the problem into two stages, connected by the head motion as an intermediate representation. EgoEgo first integrates SLAM and a learning approach to estimate accurate head motion. Subsequently, leveraging the estimated head pose as input, EgoEgo utilizes conditional diffusion to generate multiple plausible full-body motions. This disentanglement of head and body pose eliminates the need for training datasets with paired egocentric videos and 3D human motion, enabling us to leverage large-scale egocentric video datasets and motion capture datasets separately. Moreover, for systematic benchmarking, we develop a synthetic dataset, AMASS-Replica-Ego-Syn (ARES), with paired egocentric videos and human motion. On both ARES and real data, our EgoEgo model performs significantly better than the current state-of-the-art methods.

==> 4experiment_old.tex <==
\section{Experiments}
% We first introduce the datasets and evaluation metrics we used. Then we evaluate our full pipeline \textbf{EgoEgo} by comparing against two baselines (PoseReg~\cite{yuan2019ego} and Kinpoly~\cite{luo2021dynamics}) on both synthetic and real datasets using a number of metrics. In addition, we evaluate our head pose estimation approach in stage 1 and the full-body pose estimation model in stage 2. And we conduct ablation studies to showcase the effects of head pose prediction for the stage 2 model. Finally, we perform human perceptual studies for the full pipeline and the full-body pose estimation methods. 
% \subsection{Implementation Details}

\jw{I think we should reorganize the sections based on the experiments: first body from video, and then head from video, and then body from head, and then ablations and human studies (actually human studies can be merged in the first and third subsections too). For each subsection, you talk about datasets, metrics, and baselines.  Otherwise it looks very messy and hard to understand right now.}

\subsection{Datasets}

\noindent\textbf{AMASS-Replica-Ego-Syn (ARES)} is our synthetic dataset which contains synthetic egocentric videos and ground truth motions. Since no existing dataset contains large-scale paired egocentric videos and ground truth motions, we use the ARES dataset to train the baseline methods and evaluate different methods. We also use the head motion and videos provided by ARES to train our HeadNet, but do not use the ground truth body motion. ARES contains about 15 hours of motion across 18 scenes. We remove 5 scenes from training as unseen scenes. The training dataset consists of about 1.2M frames in 13 different scenes. The testing dataset contains 34, 850 frames from 5 unseen scenes. 
% The testing dataset contains 144,834 frames in 18 scenes, while 34,850 frames are from the 5 unseen scenes. 
% Notice that the motions of overlapped scenes in testing are from different mocap subsets in AMASS. Thus, all the motions in the testing dataset are unseen during training. 

\noindent\textbf{AMASS}~\cite{mahmood2019amass} is a large-scale motion capture dataset with about 45 hours of diverse motions. We use AMASS to train our full-body motion estimation model from the head pose. Since the baseline methods rely on paired egocentric video and ground truth motions, they cannot benefit from this large-scale dataset for training. 

\noindent\textbf{Kinpoly-MoCap}~\cite{luo2021dynamics} consists of egocentric videos and 3D motions captured with motion capture devices and a head-mounted camera. The total duration of the motion is about 80 minutes. Since it uses motion capture devices, the egocentric video is constrained to a single lab scene. We use the Kinpoly-MoCap dataset to evaluate different methods on real-captured images.  

\noindent\textbf{Kinpoly-RealWorld}~\cite{luo2021dynamics} contains paired egocentric videos and head poses captured using iPhone ARKit. We use this dataset to train our HeadNet used for Kinpoly-MoCap. 

\noindent\textbf{GIMO}~\cite{zheng2022gimo} consists of egocentric video, eye gaze, 3D motions, and scanned 3D scenes. This dataset is collected using Hololens, iPhone 12, and IMU-based motion capture suits to study motion prediction tasks guided by eye gaze. We use paired egocentric video and head pose from 15 scenes for training our HeadNet and use the paired egocentric video and full-body motion from 4 unseen scenes for evaluation.


\subsection{Evaluation Metrics and Baselines}
\paragraph{Evaluation Metrics.}

\begin{table}[t!]
\small
\begin{center}
%\centering
\footnotesize{
%\resizebox{2\columnwidth}{!}{
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}l||cccccc@{}} 
%\begin{tabular}{|c|c|c} 
 \toprule 
 Method     & $\mathbf{O}_{head}$ & $\mathbf{T}_{head}$ & MPJPE & Accel & FS  \\
        \midrule
        PoseReg~\cite{yuan2019ego} & 0.77 & 354.7 & 147.7 & 127.6 & 87.1 \\
        Kinpoly-OF~\cite{luo2021dynamics} & 0.62 & 323.4 & 141.6 & 7.3 & 4.2  \\
        EgoEgo (ours) & \textbf{0.20} & \textbf{148.0} & \textbf{121.1} & \textbf{6.2} & \textbf{2.7} \\
        \bottomrule
\end{tabular}
}
\end{center}
\vspace{-4mm}
\caption{Full-body motion estimation from egocentric video on ARES.} 
    \label{tab:complete_estimation_ares}
\vspace{-2mm}
\end{table}


\begin{table}[t!]
\small
\begin{center}
%\centering
\footnotesize{
%\resizebox{2\columnwidth}{!}{
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}l||cccccc@{}} 
%\begin{tabular}{|c|c|c} 
 \toprule 
 Method     & $\mathbf{O}_{head}$ & $\mathbf{T}_{head}$ & MPJPE  & Accel & FS  \\
        \midrule
        PoseReg~\cite{yuan2019ego} & 1.05 & 1943.9 & 160.4 & 61.8 & 10.8 \\
        Kinpoly-OF~\cite{luo2021dynamics} & 1.33 & 2475.5 & 230.5 & 16.4 & 15.8  \\
        EgoEgo (ours) & \textbf{0.58} & \textbf{505.1} & \textbf{125.9} & \textbf{8.0} & \textbf{1.6} \\
        \bottomrule
\end{tabular}
}
\end{center}
\vspace{-4mm}
\caption{Full-body motion estimation from egocentric video on Kinpoly-MoCap~\cite{luo2021dynamics}. } 
    \label{tab:complete_estimation_kinpoly}
\vspace{-2mm}
\end{table}



\begin{table}[t!]
\small
\begin{center}
%\centering
\footnotesize{
%\resizebox{2\columnwidth}{!}{
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}l||cccccc@{}} 
%\begin{tabular}{|c|c|c} 
 \toprule 
 Method     & $\mathbf{O}_{head}$ & $\mathbf{T}_{head}$ & MPJPE & Accel & FS \\
        \midrule
        PoseReg~\cite{yuan2019ego} & 1.51 & 1528.6 & 189.3 & 71.5 & 14.2 \\
        Kinpoly-OF~\cite{luo2021dynamics} & 1.52 & 1739.3 & 404.2 & 21.9 & 14.4  \\
        EgoEgo (ours) & \textbf{0.67} & \textbf{356.8} & \textbf{152.1} & \textbf{10.4} & \textbf{1.9} \\
        \bottomrule
\end{tabular}
}
\end{center}
\vspace{-4mm}
\caption{Full-body motion estimation from egocentric video on GIMO~\cite{zheng2022gimo}. } 
    \label{tab:complete_estimation_gimo}
\vspace{-2mm}
\end{table}

\begin{itemize}
   \vspace{-2mm}
    \item \textbf{Head Orientation Error $\left( \mathbf{O}_{head} \right)$} computes the Frobenius norm of the difference between the $3 \times 3$ rotation matrix $||\bm{R}_{pred}\bm{R}_{gt}^{-1} - \bm{I}||_{2}$, where $\bm{R}_{pred}$ is the predicted head rotation matrix and $\bm{R}_{gt}$ is the ground truth head rotation matrix. 
    \vspace{-2mm}
    \item \textbf{Head Translation Error $\left( \mathbf{T}_{head} \right)$} is computed by taking the mean Euclidean distance of two trajectories. We use this metric to measure the head joint translation errors in millimeters $\left(mm\right)$.
    \vspace{-2mm}
    \item \textbf{MPJPE} represents mean per-joint position errors in millimeters $\left(mm\right)$.  
    \vspace{-2mm}
    \item \textbf{Accel} represents the difference of acceleration between predicted joint positions and ground truth joint positions measured in $\left(mm/s^2\right)$. 
    \vspace{-2mm}
    \item \textbf{FS} represents foot skating metric and is computed following \cite{he2022nemf}. Specifically, we first project the toe and ankle joints' velocity to the $xy$ plane and compute the $L{1}$ norm of the projected velocities in each step denoted as $v_{t}$. We only accumulate the horizontal translation for those steps that have a height $h_{t}$ lower than a specified threshold $H$. And the metric is calculated as a mean of weighted values $v_{t}(2-2^{\frac{h_{t}}{H}})$ across the sequence and is measured in $\left(mm\right)$.      
\end{itemize} 


\begin{figure*}[h]
\begin{center}
\vspace{-5mm}
\includegraphics[width=0.95\textwidth]{CVPR_2023_submission/figures/Figure_last_qualitative_res.pdf}
\end{center}
\vspace{-4mm}
\caption{Qualitative results comparisons. We show the results of two egocentric videos from different scenes.}
\label{fig:qualitative_res}
\vspace{-1mm}
\end{figure*}

\vspace{-4mm}
\paragraph{Baselines for Full-Body Pose Estimation from Egocentric Video.} 
We compare our approach with two baselines PoseReg~\cite{yuan2019ego} and Kinpoly~\cite{luo2021dynamics}. \textbf{PoseReg}~\cite{yuan2019ego} takes a sequence of optical flow features as input and uses an LSTM model to predict the pose state at each time step. The pose state consists of root translation, root orientation, joint rotations, and corresponding velocities including root linear velocity and angular velocities of all the joints. \textbf{Kinpoly-OF}~\cite{luo2021dynamics} proposes a per-step regression model to estimate full body motion from optical flow features. Because our problem only allows for egocentric video as input, we choose the option of Kinpoly which only has optical flow features as input, without relying on ground truth head poses and action labels that depend on additional knowledge. The baselines are trained on ARES with paired egocentric video and ground truth motions. 

\vspace{-4mm}
\paragraph{Baselines for Full-Body Pose Estimation from GT Head Pose.}
We compare our conditional diffusion model for full-body pose estimation with two baselines AvatarPoser~\cite{jiang2022avatarposer} and Kinpoly-Head~\cite{luo2021dynamics}. \textbf{AvatarPoser}~\cite{jiang2022avatarposer} takes both head and hand pose as input to predict full body motion. We remove the hand poses from the input and modified it to a setting with head pose input only. \textbf{Kinpoly-Head}~\cite{luo2021dynamics} is our modified variant of the Kinpoly model that only takes the head pose as input. Both the baselines and our method are trained on AMASS with high-quality motion capture data. 

\subsection{Results}

\begin{table}[!t]
    \centering
    % \vspace{-5mm}
    % \vspace{-2mm}
    %\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
    %\begin{adjustbox}{width=0.9\textwidth} {
    \small
      \begin{tabular}{lcccccccc}
        \toprule
        
         & \multicolumn{2}{c}{DROID-SLAM~\cite{teed2021droid}} & 
        \multicolumn{2}{c}{Hybrid} \\
        
        \cmidrule(lr){2-3}\cmidrule(lr){4-5} 
        
        & $\mathbf{O}_{head}$  & $\mathbf{T}_{head}$ & $\mathbf{O}_{head}$  & $\mathbf{T}_{head}$  \\
        
        \midrule
        
        ARES & 0.62 & 411.3 & 0.23 & 176.5  \\
        Kinpoly & 0.55 & 1290.8 & 0.58 & 487.8 \\
        GIMO & 0.67 & 865.4 & 0.68 & 304.7 \\
        \bottomrule
       
      \end{tabular}
      %}\end{adjustbox}
    % \vspace{-0.6cm}
     \caption{Head pose estimation on testing datasets.}
    \label{tab:head_pose_estimation}
\end{table}

\begin{table}[t!]
\small
\begin{center}
%\centering
\footnotesize{
%\resizebox{2\columnwidth}{!}{
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}l||cccccc@{}} 
%\begin{tabular}{|c|c|c} 
 \toprule 
 Method     & $\mathbf{O}_{head}$ & $\mathbf{T}_{head}$ & MPJPE & Accel & FS  \\
        \midrule
        AvatarPoser~\cite{jiang2022avatarposer} & 0.19 & \textbf{28.6} & 124.7 & 16.1 & 18.8 \\
        Kinpoly-Head~\cite{luo2021dynamics} & 0.19 & 87.8 & 110.9 & 11.4 & 11.2  \\
        Diffusion Model (ours) & \textbf{0.04} & 36.7 & \textbf{109.0} & \textbf{10.5} & \textbf{4.4} \\
        \bottomrule
\end{tabular}
}
\end{center}
\vspace{-4mm}
\caption{Full-body motion estimation from GT head pose on AMASS testing dataset~\cite{luo2021dynamics}. } 
    \label{tab:stage2_estimation_amass}
% \vspace{-4mm}
\end{table}

\paragraph{Full-Body Pose Estimation from Egocentric Video.}
We compare the complete pipeline of EgoEgo with baseline methods PoseReg~\cite{yuan2019ego} and Kinpoly-OF~\cite{luo2021dynamics} on ARES, GIMO and Kinpoly datasets as shown in Table~\ref{tab:complete_estimation_ares}, Table~\ref{tab:complete_estimation_gimo} and Table~\ref{tab:complete_estimation_kinpoly} respectively. We show that our EgoEgo outperforms all the baselines by a large margin on all three datasets. We show qualitative results in Figure~\ref{fig:qualitative_res}. Our generated motions better preserve the root trajectories. And our approach can also generate more dynamic and realistic motions compared to the baselines. 
\vspace{-4mm}
\paragraph{Head Pose Estimation.}
We evaluate the head pose estimation on the three datasets as shown in Table~\ref{tab:head_pose_estimation}. We compare the prediction results of DROID-SLAM~\cite{teed2021droid} and our hybrid approach. We apply a rotation to the SLAM trajectory by aligning the first predicted head pose of SLAM with the ground truth head pose. Our hybrid approach combines the accurate rotation prediction from HeadNet and re-scaled translation of gravity-aligned SLAM results to produce more accurate head pose estimation results as input to the second stage.
\vspace{-4mm}
\paragraph{Full-Body Pose Estimation from GT Head Pose.}
We compare our proposed conditional diffusion model with our modified versions of baseline methods AvatarPoser~\cite{jiang2022avatarposer} and Kinpoly-Head~\cite{luo2021dynamics} on AMASS testing dataset as shown in Table~\ref{tab:stage2_estimation_amass}. Since our model is a generative model, there are multiple plausible predictions from the same head pose input. To compare our method quantitatively, we generate 200 samples for each head pose input and use the one with the smallest MPJPE as our result.   

\subsection{Ablation Studies} 
\paragraph{Effects of Components in Head Pose Estimation.}
We study the effects of each component in head pose estimation in Table~\ref{tab:ablation_head_pose_hybrid}. We showcase that the rotation for aligning gravity direction and the learned scale are both effective to improve head translation results. 

\begin{table}[!t]
    \centering
    % \vspace{-5mm}
    % \vspace{-2mm}
    %\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
    %\begin{adjustbox}{width=0.9\textwidth} {
    \small
    \setlength{\tabcolsep}{2pt}
      \begin{tabular}{lcccccccc}
        \toprule
        
         & \multicolumn{2}{c}{ARES} & 
        \multicolumn{2}{c}{Kinpoly} & 
        \multicolumn{2}{c}{GIMO} \\
        
        \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}  
        
        & $\mathbf{O}_{head}$  & $\mathbf{T}_{head}$ & $\mathbf{O}_{head}$  & $\mathbf{T}_{head}$ & $\mathbf{O}_{head}$  & $\mathbf{T}_{head}$  \\
        
        \midrule
        SLAM & 0.62 & 411.33 & \textbf{0.55} & 1290.82 & \textbf{0.67} & 865.41 \\
        SLAM+S & 0.62 & 325.95 & 0.55 & 643.45 & 0.67 & 569.48 \\
        SLAM+S+G & 0.62 & 176.54 & 0.55 & 487.77 & 0.67 & 304.74 \\
        Full model & \textbf{0.23} & \textbf{176.54} & 0.58 & \textbf{487.77} & 0.68 & \textbf{304.74}  \\
        \bottomrule
       
      \end{tabular}
     %  }\end{adjustbox}
    % \vspace{-0.6cm}
     \caption{Ablation study for the components in head pose estimation. S represents the scale predicted by HeadNet, and G represents GravityNet.}
    \label{tab:ablation_head_pose_hybrid}
\end{table}

\vspace{-4mm}
\paragraph{Effects of Head Pose in Full-Body Pose Estimation.}
We compare the full-body pose estimation results that take our predicted head poses and the ground truth head poses as input. Table~\ref{tab:ablation_head_pose_gt} shows that the ground truth head poses significantly improve the full body pose estimation, indicating that by developing methods that predict more accurate head pose, the full body pose estimation can be further improved.     

% \begin{table}[t!]
% \small
% \begin{center}
% %\centering
% \footnotesize{
% %\resizebox{2\columnwidth}{!}{
% \setlength{\tabcolsep}{5pt}
% \begin{tabular}{@{}l||cccccc@{}} 
% %\begin{tabular}{|c|c|c} 
%  \hline
%  Method     & $\mathbf{O}_{head}$ & $\mathbf{T}_{head}$ & MPJPE & Accel & FS  \\
%         \midrule
%         EgoEgo & 0.20 & 148.0 & 121.1 & \textbf{4.9} & \textbf{2.7} \\
%         EgoEgo w GT Heaad & \textbf{0.04} & \textbf{29.1} & \textbf{105.6} & 5.8 & 3.0 \\
%         \midrule
%         EgoEgo & 0.58 & 505.1 & 125.9 & \textbf{7.0} & \textbf{1.6} \\
%         EgoEgo w GT Heaad & \textbf{0.03} & \textbf{60.7} & \textbf{76.0} & 7.5 & 2.5 \\
%         \midrule 
%         EgoEgo & 0.67 & 356.8 & 152.1 & \textbf{4.7} & 1.9 \\
%         EgoEgo w GT Heaad & \textbf{0.06} & \textbf{66.0} & \textbf{125.7} & 5.1 & \textbf{1.7} \\
%         \bottomrule
% \end{tabular}
% }
% \end{center}
% \vspace{-4mm}
% \caption{Ablation study.} 
%     \label{tab:ablation_head_pose_gt}
% \vspace{-4mm}
% \end{table}

\begin{table}[!t]
    \centering
    % \vspace{-5mm}
    % \vspace{-2mm}
    %\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
    %\begin{adjustbox}{width=0.9\textwidth} {
    \small
    \setlength{\tabcolsep}{2pt}
      \begin{tabular}{lcccccc}
        \toprule
        
         & \multicolumn{2}{c}{ARES} & 
        \multicolumn{2}{c}{Kinpoly} & 
        \multicolumn{2}{c}{GIMO} \\
        
        \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}  
        
        & EE  & EE w GT & EE  & EE w GT &  EE  & EE w GT  \\
        
        \midrule
        $\mathbf{O}_{head}$ & 0.20 & \textbf{0.04} & 0.58 & \textbf{0.03} & 0.67 & \textbf{0.06} \\
        $\mathbf{T}_{head}$ & 148.0 & \textbf{29.1} & 505.1 & \textbf{60.7} & 356.8 & \textbf{66.0}  \\
        MPJPE & 121.1 & \textbf{105.6} & 125.9 & \textbf{76.0} & 152.1 & \textbf{125.7} \\
        Accel & \textbf{6.2} & 6.3 & 8.0 & \textbf{7.2} & 10.4 & \textbf{10.2}  \\
        FS & \textbf{2.7} & 3.0 & \textbf{1.6} & 2.5 & 1.9 & \textbf{1.7}  \\
        \bottomrule
       
      \end{tabular}
     %  }\end{adjustbox}
    % \vspace{-0.6cm}
     \caption{Ablation study for the effects of head pose. EE represents EgoEgo.}
    \label{tab:ablation_head_pose_gt}
\end{table}


\begin{figure}[t!]
\begin{center}
\vspace{-2mm}
\includegraphics[width=0.45\textwidth]{CVPR_2023_submission/figures/Figure_human_study.pdf}
\end{center}
\vspace{-6mm}
  \caption{Results of human perceptual studies. The numbers shown in the chart represent \%.}
  % \vspace{-10mm}
  \label{fig:human_study}
\vspace{-1mm}
\end{figure}

\subsection{Human Perceptual Study}
We also conduct two human perceptual studies as part of the evaluation. The first is to evaluate the quality of predicted full-body motion from egocentric video, the second is to evaluate the quality of predicted full-body motion from ground truth head poses. In both studies, we compare four types of motion: results from our \model and from two baselines, as well as the ground truth. Each time, users are presented with two motions and asked to select which one is more plausible. Because there are 10 examples and the two motions can be from four sources, we have 60 questions for each study. Each question was answered by 20 Amazon Mechanical Turk workers. 

%We also run a human perceptual study for the full-body motion estimation methods from ground truth head poses to evaluate the motion quality of each approach. 
%\jw{I don't understand the previous sentence and feel we don't need it anyway, so I commented it out. Please double check.} For each of the 10 examples in the study, 
\jw{can you add (a) and (b) to Figure 6.} As shown in Figure~\ref{fig:human_study}(a), for full-body estimation from egocentric video, our results are preferred by 98\% and 69\% of workers when compared to the baselines. Also, when compared with the ground truth, 34\% of the responses prefer our results (note that a perfect output would achieve 50\%), suggesting that people cannot easily distinguish our results from ground truth motions. As shown in Figure~\ref{fig:human_study}(b), for full-body estimation from head poses, our results are preferred by 88\% and 79\% of workers when compared to the baselines.





